A Probabilistic Theory of Deep Learning

A grand challenge in machine learning is the development of computational algorithms that match or outperform humans in perceptual inference tasks that are complicated by nuisance variation. For instance, visual object recognition involves the unknown object position, orientation, and scale in object recognition while speech recognition involves the unknown voice pronunciation, pitch, and speed. Recently, a new breed of deep learning algorithms have emerged for high-nuisance inference tasks that routinely yield pattern recognition systems with near- or super-human capabilities. But a fundamental question remains: Why do they work? Intuitions abound, but a coherent framework for understanding, analyzing, and synthesizing deep learning architectures has remained elusive. We answer this question by developing a new probabilistic framework for deep learning based on the Deep Rendering Model: a generative probabilistic model that explicitly captures latent nuisance variation. By relaxing the generative model to a discriminative one, we can recover two of the current leading deep learning systems, deep convolutional neural networks and random decision forests, providing insights into their successes and shortcomings, as well as a principled route to their improvement.

==> ReprInvariance-Summary.tex <==
%% summary of i-Theory

\emph{Representational invariance and selectivity (RI)} are important ideas that have developed in the computational neuroscience community.
According to this perspective, the main purpose of the feedforward aspects of visual cortical processing in the ventral stream are to compute a representation for a sensed image that is invariant to irrelevant transformations (e.g., pose, lighting etc.) \cite{Pinto:2008bo,DiCarlo:2012em}. In this sense, the RI perspective is quite similar to the DRM in its basic motivations. However, the RI approach has remained qualitative in its explanatory power until recently, when a theory of invariant representations in deep architectures --- dubbed \emph{i-theory} ---  was proposed \cite{Anselmi:2007ke,PoggioOnInvariance}. Inspired by neuroscience and models of the visual cortex, it is the first serious attempt at explaining the success of deep architectures, formalizing intuitions about invariance and selectivity in a rigorous and quantitatively precise manner. 

%However, \ith has an important limitation. 
%In particular, many of its results can be understood more naturally from the probabilistic generative modeling approach presented here. We will outline a few key similarities and differences here, leaving a more detailed discussion for future work.
%The DRM-based approach -- as it provides an explicit generative model -- makes more specific testable predictions. Our results subsume their predictions and explanations, while also yielding a natural probabilistic explanation for cortical structure. Given the simplicity of the theory and its explanatory power, we believe this is a promising direction for future theoretical work in computational neuroscience.

%\subsubsection{Representations as Group Averages}
%The main equations of the RI approach map directly onto our approach, and we achieve yet another satisfying translation between perspectives:
%\begin{align*}
%	\mu_k^n(I) &= \frac{1}{|G|} \sum_{g \in G} ( \langle gT^k | I \rangle)^n  \\
%	a^2(I)         &=  \frac{1}{|G|} \sum_{g \in G} \exp( \langle W(c,g) | I \rangle)  \\
%	                  &=  \frac{1}{|G|} \sum_{g \in G} \sum_{n \in \N} \frac{1}{n!}( \langle W(c,g) | I  \rangle )^n \\
%	p(c|I)      &\propto \frac{1}{|G|} \sum_{g \in G} \exp( \ln p(c | I, g) ) \\
%	                 &= \frac{1}{|G|} \sum_{g \in G} \sum_{n \in \N} \frac{1}{n!}( \ln p(I | c, g] )^n	                  
%\end{align*}
%Thus if we make the correspondence $k \leftrightarrow c,\, gT^k \leftrightarrow W(c,g) \leftrightarrow \ln p(I|c,g), \sum_n \frac{1}{n!}\mu_k^n(I) \leftrightarrow p(c|I)$  we can re-interpret all quantities in \ith as Bayesian probabilistic quantities. Indeed, it is clear that there is actually much more freedom in the RI perspective as the $\mu_n^k(I)$ are not constrained so that the sum over $n \in \N$ yields a series approximation to the $\exp(\cdot)$ function. Thus, in order to execute proper probabilistic message passing, the network is forced to re-learn the weights such that the $\frac{1}{n!}$ weights yield proper probabilities. The probabilistic perspective, on the other hand, makes it explicit and show that no other choices for the weights are consistent with a proper probabilistic message passing interpretation.

The \ith posits a representation that employs group averages and orbits to explicitly insure invariance to specific types of nuisance transformations. These transformation must possess a mathematical semi-group structure; as a result, the invariance constraint is relaxed to a notion of partial invariance, which is built up slowly over multiple layers of the architecture.

At a high level, the DRM shares similar goals with \ith in that it attempts to capture explicitly the notion of nuisance transformations. However, the DRM differs from \ith in two critical ways. First, it does not impose a semi-group structure on the set of nuisance transformations. This provides the DRM the flexibility to learn a representation that is invariant to a wider class of nuisance transformations, including non-rigid ones. Second, the DRM does not fix the representation for images in advance. Instead, the representation emerges naturally out of the inference process. For instance, sum- or max-pooling emerge as probabilistic marginalization over nuisance variables and thus are necessary for proper inference. The deep iterative nature of the DCN also arises as a direct mathematical consequence of the DRM's rendering model, which comprises multiple levels of abstraction.

This is the most important difference between the two theories. Despite these differences, \ith is complementary to our own in several ways, one of which is that it spends a good deal of energy focusing on questions such as: How many templates are required for accurate discrimination? How many samples are needed for learning? We plan to pursue these questions for the DRM in future work.

%\subsubsection{Achieving Invariance by using Templates in Memory}
%In order to estimate the correct class posterior, we need to consider all possible hypotheses for objects and poses. Thus, we need to store in memory either all possible images of an object or all possible templates. The latter is preferred because it allows us to recognize new objects with only one or a few observations (One-Shot Learning). From the DRM's perspective, class appearance models are simply factorized products of nuisance transformations that approximate the rendering process. The templates then acquire a meaning as partial inversions of local nuisance transformations, as formalized in Eq.~\ref{eqn:FwdProp}. 
%
%\subsubsection{Multi-View Templates and Class-specific Transformations}
%Of course, for larger nuisances $\Delta g$, we require a new template, and thus a new bin $G_{b+}$. In this way, we can naturally arrive at multiple-view stored template strategy, wherein we store in memory many different views of the same object (sufficiently spaced apart so that the binning is as coarse as possible), and test for the object and view by template matching against these views. Indeed, this strategy is well-known to exist in the face areas of macaques and humans, where many different views of faces are stored, and view-independence built up by pooling over ranges (bins) of these views \cite{Tsao, DiCarlo}.
%
%Further developing this line of thinking, we can consider different classes of objects and the different kinds of transformations they allow for. For example, rigid boxes have a set of transformations $G_{box}$, whereas faces can undergo a far richer set of transformations (expressions), $G_{face}$. Since the DRM can handle a prior $p(g|c)$, \emph{it naturally allows for class-specific transformations i.e. the existence of face areas and rigid box areas}. There is no need to postulate specialized mechanisms for different classes, unless of course certain objects have enormous ethological value (as faces do).
%
%\subsubsection{Embedding Dimension} 
%Given a binning $g \in \G=\cup_b \G_b$, we can now use the histogram over bins to partition an object's orbit (under the group action) into a single interval or a few spaced intervals, as described. Then in this new space (where points represent sections of object orbits), we can apply Johnson-Lindenstrauss Lemma to compute the minimum embedding dimensions required for discrimination and compare it to that derived from the RI framework:
%\begin{align*}
%	d_{\textrm{min}}^{\textrm{DRM}} &= \frac{c}{\epsilon^2} ( \ln(|\Cl|) + \ln |\mathcal{B}|) \\
%	d_{\textrm{min}}^{\textrm{\ith}} &= \frac{c}{\epsilon^2}  \ln(|\mathcal{I}|)
%\end{align*}
%where $|\mathcal{I}|$ is the total number of images in the training set. Note that, again, we have reduced the number of pose-tests by increasing the complexity of the template match to be robust to small changes in the pose, $g \in \G_b$. Clearly, $d_{\textrm{min}}^{\textrm{Bayes}} < d_{\textrm{min}}^{\textrm{RI}}$ by a factor that is $O(\ln |\G_b|)$.
%
%\subsubsection{How many templates are required for accurate discrimination?}
%The second strategy for reducing the computational burden was reducing the total number of templates, $\mathcal{T}$. If there is significant shared intensity variation amongst the appearances of different objects, then we expect that $|\mathcal{T}| \ll |\Cl|$, or more generally, $|\mathcal{T}| |\G| \ll |\Cl| |G|$.
%Thus, we have motivated the need for a \emph{template basis}: a set of templates that can be combined to form approximations to the input image (patch). Such templates need not be images of objects or object parts per se; indeed they can be highly non-intuitive when visualized \cite{Krizhevsky:2012wl}. This is also seen empirically one of the most powerful and widely used models for natural image patches: Gaussian Mixture models (GMMs) \cite{Zoran-Weiss:2013pr}.
%
%Regardless of the model used, one must estimate the number of templates required for accurate discrimination/recognition of objects. In this vein, we use the approach outlined above, in conjunction with Johnson-Lindenstrauss Lemma, to determine the minimum number of templates needed.
%


==> abstract_arXiv_v1.tex <==
%auto-ignore
A grand challenge in machine learning is the development of computational algorithms that match or outperform humans in perceptual inference tasks that are complicated by nuisance variation. For instance, visual object recognition involves the unknown object position, orientation, and scale in object recognition while speech recognition involves the unknown voice pronunciation, pitch, and speed. Recently, a new breed of deep learning algorithms have emerged for high-nuisance inference tasks that routinely yield pattern recognition systems with near- or super-human capabilities. But a fundamental question remains: Why do they work? Intuitions abound, but a coherent framework for understanding, analyzing, and synthesizing deep learning architectures has remained elusive. We answer this question by developing a new probabilistic framework for deep learning based on the {\em Deep Rendering Model}: a generative probabilistic model that explicitly captures latent nuisance variation. By relaxing the generative model to a discriminative one, we can recover two of the current leading deep learning systems, deep convolutional neural networks and random decision forests, providing insights into their successes and shortcomings, as well as a principled route to their improvement.
